Geometry of Deep Generative Models for Disentangled Representations

Deep generative models like variational autoencoders approximate the intrinsic geometry of high dimensional data manifolds by learning low-dimensional latent-space variables and an embedding function. The geometric properties of these latent spaces has been studied under the lens of Riemannian geometry; via analysis of the non-linearity of the generator function. In new developments, deep generative models have been used for learning semantically meaningful `disentangled' representations; that capture task relevant attributes while being invariant to other attributes. In this work, we explore the geometry of popular generative models for disentangled representation learning. We use several metrics to compare the properties of latent spaces of disentangled representation models in terms of class separability and curvature of the latent-space. The results we obtain establish that the class distinguishable features in the disentangled latent space exhibits higher curvature as opposed to a variational autoencoder. We evaluate and compare the geometry of three such models with variational autoencoder on two different datasets. Further, our results show that distances and interpolation in the latent space are significantly improved with Riemannian metrics derived from the curvature of the space. We expect these results will have implications on understanding how deep-networks can be made more robust, generalizable, as well as interpretable.

==> Sections/Part1.tex <==


\subsection{\cite{Szabo_2017}}

\subsection{Conditional Generative Model with Adversarial Training}

==> Sections/PreviousWork.tex <==
Over the last decade, there has been an increased interest in understanding the geometry of neural networks. Several papers like \cite{Brahma2016} have focused on providing theoretical insights and justification behind the success of deep learning models. With the current success of deep generative models like GANs and VAEs in various applications like realistic image generation \cite{DCGAN_2015}, learning interpretable features \cite{Szabo_2017,Mathieu_2016} and unsupervised domain adaptation \cite{DANN}, geometric understanding of these models have received attention. Several recent works have focused on establishing the geometry of generative models \cite{Hauberg_2017,Kuhnel2018,Shao2018,Laine2018}. Shao et al. \cite{Shao2018} suggest that the generated Riemannian data manifold generated by a VAE, while nonlinear has very low curvature. This conclusion further implies that the linear movements in the latent space result in movements approximately along the geodesics of the generated data manifold. %Thus a Riemannian manifold on the latent space is defined by the generator mapping function $f(Z)$. 
Thus, statistics computed on a much smaller dimensional latent space, can be used along with the Riemannian geometry induced by the generator mapping function $f(Z)$, to draw inferences in the high dimensional data manifold. Later, \cite{Hauberg_2017,Kuhnel2018} showed that the latent space is typically nonlinear and computations should appropriately account for its curvature.

While these works address the geometry of latent space of deep generative modes, the analysis has usually been limited to latent space of one generative model \emph{i.e.} VAEs. In this work, we extend the analysis to  generative models for disentangled representation learning.

% \begin{itemize}
% \item Briefly talk about geometry in deep networks
% \item Categorization of geometry in deep nets
% \item Motivate for generative model geometrical analysis
% \item Discuss the 4 papers
% \end{itemize}
 

==> Sections/curvature.tex <==
\begin{table}[h!]
{\small 
	\centering
		\begin{tabular}{|c|cc|cc|cc|}
		\hline
        Models & \multicolumn{2}{c|}{Specified} & \multicolumn{2}{c|}{Unspecified} & \multicolumn{2}{c|}{Combined} \\\cline{2-7}
 & Margin & Curvature &Margin & Curvature & Margin & Curvature \\ \hline
\cite{Szabo_2017} & $1.59\times 1e^{-4}$& 0.0348 & 0 & -&& \\\hline
\cite{Mathieu_2016} & $1.61 \times 1e^{-4}$&0.0293&  $1.262 \times 1e^{-4}$& 0.043&& \\\hline
\cite{Jha_2018} && & & &&\\\hline
	\end{tabular}
	\caption{MNIST digits}
	\label{tab: 5k_results_mnist}
}
\end{table}

==> Sections/d_vs_c.tex <==
\begin{center}
\begin{tabular}{|c|c|c|c|} 
 \hline
 Dimension & 16 & 64 & 80 \\\hline 
 Curvature  & & & \\ \hline
 NMI score  & 54 & 55 & 57 \\ \hline
 \end{tabular}
 \end{center}

==> Sections/r_vs_e_comb.tex <==
 \begin{table*}[ht!]
\centering
\begin{tabular}{|c|c|c|c|c||c|c|c|} 
 \hline
 & Models & Szabo \emph{et al}& Mathieu \emph{et al.} & Jha \emph{et al.} & Szabo \emph{et al}& Mathieu \emph{et al.} & Jha \emph{et al.} \\\hline 
Distances  &Euclidean  & 0.114 & 0.112 & 0.116 \\\cline{2-5}
  &Riemannian & 0.297 & 0.355 & 0.336 \\\hline
 Clustering & Euclidean & 91.12 & 94.32 & 92.22 \\\cline{2-5}
  F score& Riemannian & 94.56 & 98.00 & 96.60 \\\hline 
 \end{tabular}
 \caption{MNIST dataset: Comparison of Average distance between randomly selected 100 pairs and clustering performance performance: Riemannian Distance vs Euclidean Distance. The large differences in the distance/ F score is a result of curvature in the latent space.}
 \label{tab: r_e_mnist}
\end{table*}

==> Sections/unspecified_c.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Dataset & VAE & Szabo \emph{et al.}& Mathieu  \emph{et al.}& Jha \emph{et al.}\\\hline
MNIST & 0.216 & 0.290 & 0.309 & 0.301 \\\hline
\end{tabular}
\caption{Comparison of $\hat{c}$ values for unspecified space of different disentangling models with VAE for MNIST digits.}
\label{tab: un_c_value}
\end{table}
